Semantic Summarization of Egocentric Photo Stream Events

With the rapid increase of users of wearable cameras in recent years and of the amount of data they produce, there is a strong need for automatic retrieval and summarization techniques. This work addresses the problem of automatically summarizing egocentric photo streams captured through a wearable camera by taking an image retrieval perspective. After removing non-informative images by a new CNN-based filter, images are ranked by relevance to ensure semantic diversity and finally re-ranked by a novelty criterion to reduce redundancy. To assess the results, a new evaluation metric is proposed which takes into account the non-uniqueness of the solution. Experimental results applied on a database of 7,110 images from 6 different subjects and evaluated by experts gave 95.74% of experts satisfaction and a Mean Opinion Score of 4.57 out of 5.0. Source code is available at https://github.com/imatge-upc/egocentric-2017-lta

==> 3_1_segmentation.tex <==
\subsection{Event Segmentation with R-clustering} \label{sec:segmentation}

Recently, Talavera et al. \cite{talavera2015r} proposed a temporal segmentation algorithm for image sequences captured through a low-temporal resolution camera. Their method focuses on what the camera wearer sees and aims at grouping together images that looks similar. Image appearance is encoded by global CNN features computed using ImageNet as a fixed feature extractor. This computes a 4096-D vector for every image that contains the activations of the hidden layer immediately before the last fully-connected layer, corresponding to the classifier. Since the ConvNet has been pre-trained on a large database of objects, and the images capture scenes composed of objects, the global CNN features give a good holistic representation of image appearance. %To reduce the dimensionality of the data and their large variations, their are normalized \cite{talavera2015r} prior to apply PCA.
Based on this image representation, the proposed algorithm puts together two different approaches for temporal segmentation with complementary properties:  ADaptative WINdowing (ADWIN) that applied to segment the video (look bellow) tends to undersegment the video, and Agglomerative Clustering (AC), that typically leads to oversegmentation of the egocentric data. The R-clustering combines both techniques in an energy-minimization framework that is able to produce a smoothed and temporally coherent segmentation of the egocentric collection of images.

\subsubsection{Under-segmentation}
ADWIN is a change detector that gives a rigorous guarantee of the performances in term of controlled number of false alarms. 
Given two temporally adjacent (sub)windows of the data, say $W_1$ and $W_2$ ($W = W_1 \cup W_2$), ADWIN iteratively checks if their empirical means are above a threshold. For a $k-$dimensional signal  \cite{Drozdzal2014}, the threshold is computed as
$$\epsilon_{cut} = k^{1/p}\sqrt{\frac{1}{2m}\ln\frac{4}{k\delta'}}$$, where $p$ indicates the $p-$norm, $\delta \in (0, 1)$ is a user defined confidence parameter normalized by the length of $W$ and $m$ is the harmonic mean of the lengths of the two subwindows.
From the above formula, it can be deduced that ADWIN is unable to predict changes involving a relatively small number of samples, changes that are not strong enough given the dimensionality of the data, and changes due to higher order statistics. For all these reasons, it usually leads to under-segmentation. 

\subsubsection{Over-segmentation}
AC works by iteratively grouping the most similar clusters in a bottom-up fashion until a pre-determined criterion, typically a threshold on the cluster consistency, is fitted. 

\subsubsection{Fusion}
 automatically finds a trade-off between the undersegmentation provided by ADWIN and the oversegmentation  provided by AC in a Graph Cut energy-minimization framework using two unary terms for both AC and ADWIN and a binary term to force  events boundaries to be abrupt (?!?!?!).





==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges
		
